Automated Reasoning in Normative Detachment Structures with Ideal Conditions

Systems of deontic logic suffer either from being too expressive and therefore hard to mechanize, or from being too simple to capture relevant aspects of normative reasoning. In this article we look for a suitable way in between: the automation of a simple logic of normative ideality and sub-ideality that is not affected by many deontic paradoxes and that is expressive enough to capture contrary-to-duty reason- ing. We show that this logic is very useful to reason on normative scenarios from which one can extract a certain kind of argumentative structure, called a Normative Detachment Structure with Ideal Conditions. The theoretical analysis of the logic is accompanied by examples of automated reasoning on a concrete legal text.

==> phead.tex <==

\newcommand{\Id}{\texttt{I}}
\newcommand{\SId}{\texttt{A}}
\newcommand{\Ob}{\texttt{O}}

\newcommand{\kll}{\texttt{kill}}
\newcommand{\gtl}{\texttt{gently}}

\newcommand{\hlp}{\texttt{help}}
\newcommand{\tll}{\texttt{tell}}

%%%%%%%%%%%%%
% FPC
%%%%%%%%%%%%%
\newcommand{\fpc}{FPC\xspace}
\newcommand{\eprover}{\textsf{E-prover}\xspace}
\newcommand{\tptp}{TPTP\xspace}
\newcommand{\ocaml}{OCaml\xspace}
\newcommand{\lpro}{$\lambda$Prolog\xspace}
\newcommand{\linux}{Linux\xspace}
\newcommand{\pcert}{ProofCert\xspace}


%%%%%%%%%%%%%
% Utilities
%%%%%%%%%%%%%

\newcommand{\lP}{$\lambda$Prolog\xspace}
\newcommand{\zc}[1]{{\color[rgb]{1.000000,0.509804,0.278431} ZC: #1}}
\newcommand{\dm}[1]{{\color[rgb]{0.45, 0.31, 0.59} DM : #1}}
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\lpInf}{\: \turnstyle \:}
\newcommand{\turnstyle}{\hbox{\tt \ :-\ }} % turnstyle Prolog-style

%%%%%%%%%%%%%%
% System names
%%%%%%%%%%%%%%
\newcommand\proofsystem[1]{\mbox{\slshape #1}\xspace}
\newcommand\LK   {\proofsystem{LK}}
\newcommand\LKF  {\proofsystem{LKF}}
\newcommand\LMF  {\proofsystem{LMF}}
\newcommand\aLKF {\hbox{\proofsystem{LKF}\kern-2pt$^a$}\xspace}
\newcommand\lmfa {\hbox{\proofsystem{LMF}\kern-2pt$^a$}\xspace}
\newcommand\LKU  {\proofsystem{LKU}}
\newcommand\LJ   {\proofsystem{LJ}}
\newcommand\LJF  {\proofsystem{LJF}}
\newcommand\aLJF {\hbox{\proofsystem{LJF}\kern-2pt$^a$}\xspace}
\newcommand\LKpos{\proofsystem{LKpos}}
\newcommand\LKneg{\proofsystem{LKneg}}

% Clean redefined macros (talk of oct 15th)
% Previous commands are still active(see bellow) for retrofitting : They only
% call on the new ones and should be removed.

% Naming convention:
% binary connectives [k|j][n|p][and|or]
% Unary connectives [k|j][some|all]
% Bureau :
%          simple naming          : <Connective_name>[c|e]
%          Usage (with parameters : <Connective_name>[c|e]u
% I know for LKF [c|e] is subsumed by [n|p] but this way it's more coherant

% Explore the idea of naming release with an uparrow, decide with a down arrow.

%%%%%%%%%%%%%%
% LKF Macros
%%%%%%%%%%%%%%

% => Sequents
\newcommand{\async}[2]{\vdash#1\mathbin{\Uparrow} #2}
\newcommand{\sync }[2]{\vdash#1\mathbin{\Downarrow} #2}
\newcommand{\asyncr}[4]{#1\vdash_{#2}#3\mathbin{\Uparrow} #4}
\newcommand{\syncr }[4]{#1\vdash_{#2}#3\mathbin{\Downarrow} #4}
\newcommand{\Async}[3]{#1\async{#2}{#3}}  % With Xi
\newcommand{\Sync }[3]{#1\sync{#2}{#3}}  % With Xi

% => Connectives and rules
% ==> Names
%\newcommand{\knand}{ \& }
\newcommand{\knand}{ \jnand }
%\newcommand{\knor}{\parr }
\newcommand{\knor}{\vee^{-}}
%\newcommand{\kpand}{\otimes}
\newcommand{\kpand}{\jpand}
%\newcommand{\kpor}{\oplus }
\newcommand{\kpor}{\veep }
%\newcommand{\ksome}{\Sigma }
\newcommand{\ksome}{\jsome }
%\newcommand{\kall}{\Pi }
\newcommand{\kall}{\jall}
%\newcommand{\kpfalse}{0}
\newcommand{\kpfalse}{\pfalse}
\newcommand{\kptrue}{\ptrue}
\newcommand{\knfalse}{\nfalse}
\newcommand{\kntrue}{\ntrue}
% -- Structural
\newcommand{\kstore}{\mathscr{S}}
\newcommand{\kdecide}{\mathscr{D}}
\newcommand{\krelease}{\mathscr{R}}
\newcommand{\kinit}{\mathscr{I}}
% ==> Usage
\newcommand{\initos}{init_{OS}}
\newcommand{\boxos}{{\square_{OS}}}
\newcommand{\knandu}[2]{#1 \knand #2}
\newcommand{\knoru}[2]{#1 \knor #2}
\newcommand{\kpandu}[2]{#1 \kpand #2}
\newcommand{\kporu}[2]{#1 \kpor #2}
\newcommand{\ksomeu}[1]{\ksome #1}
\newcommand{\kallu}[1]{\kall #1}


% => Bureau
%% ==> Names
\newcommand{\knandc}{\knand_c}
\newcommand{\knorc}{\knor_c}
\newcommand{\kpande}{\kpand_e}
\newcommand{\kpore}{\kpor_e}
\newcommand{\ksomee}{\ksome_e}
\newcommand{\kallc}{\kall_c}
\newcommand{\kptruee}{\kptrue_e}
\newcommand{\knfalsec}{\knfalse_c}
%--Structural
\newcommand{\kstorec}{\kstore_c}
\newcommand{\kdecidee}{\kdecide_e}
\newcommand{\kreleasee}{\krelease_e}
\newcommand{\kinite}{\kinit_e}

%% ==> Usage (with parameters)
% ZC : still not sure about giving the formula as a parameter
\newcommand{\knandcu}[4]{\knandc(#1,#2,#3,#4)} % C F C1 C2
\newcommand{\knorcu}[3]{\knorc(#1,#2,#3)} % C F C'
\newcommand{\kpandeu}[4]{\kpande(#1,#2,#3,#4)} % C F C1 C2
\newcommand{\kporeu}[4]{\kpore(#1,#2,#3,#4)} % C F Choice C'
\newcommand{\ksomeeu}[4]{\ksomee(#1,#2,#3,#4)} % C F Witness C'
\newcommand{\kallcu}[3]{\kallc(#1,#2,#3)} % C F (x\C')
\newcommand{\kptrueeu}[1]{\kptruee(#1)}
\newcommand{\knfalsecu}[2]{\knfalsec(#1,#2)}
%--Structural
\newcommand{\kstorecu}[4]{\kstorec(#1,#2,#3,#4)} %C F Indx C'
\newcommand{\kdecideeu}[3]{\kdecidee(#1,#2,#3)} % C Indx C'
\newcommand{\kreleaseeu}[3]{\kreleasee(#1,#2,#3)} % C F C'
\newcommand{\kiniteu}[3]{\kinite(#1,#2,#3)} %C F I

%%%%%%%%%%%%%%
% LJF Macros
%%%%%%%%%%%%%%
% => Sequents

\newcommand{\Rscr}{{\cal R}} % Used for an ambiguous rhs

%\newcommand{\jUnf}[4]{#1 ; #2 \vdash  #3 ; #4}% unfocused sequent
\newcommand{\jUnf}[4]{#1 \mathbin\Uparrow #2 \vdash  #3 \mathbin\Uparrow #4}% unfocused sequent
\newcommand{\jUnfamb}[3]{#1 \mathbin\Uparrow #2 \vdash  #3 \Rscr}% unfocused sequent
%\newcommand{\jUnfG}[2]{\jUnf{\Gamma}{#1}{#2}{{\cdot}}}% unf sequ with \Gamma
\newcommand{\jUnfG}[2]{\jUnf{\Gamma}{#1}{#2}{{}}}% unf sequ with \Gamma
\newcommand{\jUnfGamb}[1]{\Gamma\mathbin\Uparrow #1\vdash \Rscr}% unf sequ with \Gamma
\newcommand{\jLf}[3]{#1 \Downarrow #2 \vdash #3}% left focused sequent
\newcommand{\jLfG}[1]{\jLf{\Gamma}{#1}{R}}% left foc seq with \Gamma
\newcommand{\jRf}[2]{#1 \vdash #2 \Downarrow}% right focused sequent
\newcommand{\jRfG}[1]{\jRf{\Gamma}{#1}}% right foc seq with \Gamma
%\newcommand{\jC}[2]{{\blue {#1 \colon\,}} #2} % Use for all other instances
\newcommand{\jC}[2]{{\blue {#1 \colon}} #2} % Use for all other instances

% => Connectives
% ==> Names
\newcommand{\jarr}{\supset}
\newcommand{\jor}{\vee}
\newcommand{\jpand}{\wedge^{\scriptscriptstyle +}}
\newcommand{\jnand}{\wedge^{\scriptscriptstyle -}}
\newcommand{\jsome}{\exists}
\newcommand{\jall}{\forall}
\newcommand{\jtrue}{\hbox{\sl t}}
\newcommand{\jfalse}{\hbox{\sl f}}
% -- Strructural

\newcommand{\jinit}{\mathbb{I}}
\newcommand{\jrelease}{\mathbb{R}}
\newcommand{\jdecide}{\mathbb{D}}
\newcommand{\jstore}{\mathbb{S}}
%--
\newcommand{\jinitl}{\jinit^l}
\newcommand{\jreleasel}{\jrelease^l}
\newcommand{\jdecidel}{\jdecide^l}
\newcommand{\jstorel}{\jstore^l}

\newcommand{\jinitr}{\jinit^r}
\newcommand{\jreleaser}{\jrelease^r}
\newcommand{\jdecider}{\jdecide^r}
\newcommand{\jstorer}{\jstore^r}
% ==> Usage
\newcommand{\jarru}[2]{#1 \jarr #2}
\newcommand{\joru}[2]{#1 \jor #2}
\newcommand{\jpandu}[2]{#1 \jpand #2}
\newcommand{\jnandu}[2]{#1 \jnand #2}
\newcommand{\jsomeu}[1]{\jsome #1}
\newcommand{\jallu}[1]{\jall  #1}

% => Bureau
% ==> Names
\newcommand{\jarrc}{\jarr_c}
\newcommand{\jarre}{\jarr_e}
\newcommand{\jorc}{\jor_c}
\newcommand{\jore}{\jor_e}
\newcommand{\jpandc}{\jpand_c}
\newcommand{\jpande}{\jpand_e}
\newcommand{\jnandc}{\jnand_c}
\newcommand{\jnande}{\jnand_e}
\newcommand{\jsomec}{\jsome_c}
\newcommand{\jsomee}{\jsome_e}
\newcommand{\jallc}{\jall_c}
\newcommand{\jalle}{\jall_e}

\newcommand{\jtruec}{\jtrue_c}
\newcommand{\jtruee}{\jtrue_e}
\newcommand{\jfalsec}{\jfalse_c}
%-- Structural
\newcommand{\jinitle}{\jinitl_e}
\newcommand{\jreleasele}{\jreleasel_e}
\newcommand{\jdecidele}{\jdecidel_e}
\newcommand{\jstorelc}{\jstorel_c}

\newcommand{\jinitre}{\jinitr_e}
\newcommand{\jreleasere}{\jreleaser_e}
\newcommand{\jdecidere}{\jdecider_e}
\newcommand{\jstorerc}{\jstorer_c}

%==>Usage
% (#1,#2) [2]
\newcommand{\jarrcu}[3]{\jarrc(#1,#2,#3)}
\newcommand{\jarreu}[4]{\jarre(#1,#2,#3,#4)}
\newcommand{\jorcu}[4]{\jorc(#1,#2,#3,#4)}
\newcommand{\joreu}[4]{\jore(#1,#2,#3,#4)}
\newcommand{\jpandcu}[3]{\jpandc(#1,#2,#3)}
\newcommand{\jpandeu}[4]{\jpande(#1,#2,#3,#4)}
\newcommand{\jnandcu}[4]{\jnandc(#1,#2,#3,#4)}
\newcommand{\jnandeu}[4]{\jnande(#1,#2,#3,#4)}
\newcommand{\jsomecu}[3]{\jsomec(#1,#2,#3)}
\newcommand{\jsomeeu}[4]{\jsomee(#1,#2,#3,#4)}
\newcommand{\jallcu}[3]{\jallc(#1,#2,#3)}
\newcommand{\jalleu}[4]{\jalle(#1,#2,#3,#4)}

\newcommand{\jtruecu}[2]{\jtruec(#1,#2)}
\newcommand{\jtrueeu}[1]{\jtruee(#1)}
\newcommand{\jfalsecu}[1]{\jfalsec(#1)}
%-- Structural
\newcommand{\jinitleu}[1]{\jinitle(#1)}
\newcommand{\jreleaseleu}[3]{\jreleasele(#1,#2,#3)}
\newcommand{\jdecideleu}[3]{\jdecidele(#1,#2,#3)}
\newcommand{\jstorelcu}[4]{\jstorelc(#1,#2,#3,#4)}

\newcommand{\jinitreu}[2]{\jinitre(#1,#2)}
\newcommand{\jreleasereu}[3]{\jreleasere(#1,#2,#3)}
\newcommand{\jdecidereu}[2]{\jdecidere(#1,#2)}
\newcommand{\jstorercu}[3]{\jstorerc(#1,#2,#3)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Old ones  Should call on the new ones and be slowly eliminated.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\jeArr}[3]{\supset_e (#1,#2,#3)}
\newcommand{\jeOr}[3]{\vee_e (#1,#2,#3)}
\newcommand{\jeAndP}[3]{\wedgep_e (#1,#2,#3)}
\newcommand{\jeDelayP}[2]{\posdop_e (#1,#2)}
\newcommand{\jeAndN}[3]{\wedgen_e (#1,#2,#3)}
\newcommand{\jeDelayN}[2]{\negdop_e (#1,#2)}
\newcommand{\jeTrueP}[1]{\ptrue_e (#1)}
\newcommand{\jeSome}[3]{\exists_e(#1,#2,#3)}
\newcommand{\jeAll}[3]{\forall_e(#1,#2,#3)}

\newcommand{\jcArr}[2]{\supset_c(#1,#2)}
\newcommand{\jcOr}[3]{\vee_c (#1,#2,#3)}
\newcommand{\jcFalse}[1]{\pfalse_c (#1)}
\newcommand{\jcAndP}[2]{\wedgep_c(#1,#2)}
\newcommand{\jcDelayP}[2]{\posdop_c(#1,#2)}
\newcommand{\jcAndN}[3]{\wedgen_c(#1,#2,#3)}
\newcommand{\jcDelayN}[2]{\negdop_c(#1,#2)}
\newcommand{\jcTrueN}[1]{\ntrue_c(#1)}
\newcommand{\jcTrueP}[2]{\ptrue_c(#1,#2)}
\newcommand{\jcSome}[2]{\exists_c(#1,#2)}
\newcommand{\jcAll}[2]{\forall_c(#1,#2)}
% Structural
\newcommand{\jeDecL}[3]{\hbox{\sl DecideL}_e(#1,#2,#3)}
\newcommand{\jeDecR}[2]{\hbox{\sl DecideR}_e(#1,#2)}
\newcommand{\jeRelL}[2]{\hbox{\sl ReleaseL}_e(#1,#2)}
\newcommand{\jeRelR}[2]{\hbox{\sl ReleaseR}_e(#1,#2)}
\newcommand{\jcStoreL}[3]{\hbox{\sl StoreL}_c(#1,#2,#3)}
\newcommand{\jcStoreR}[2]{\hbox{\sl StoreR}_c(#1,#2)}
% Identity experts
\newcommand{\jeInitL}[1]{\hbox{\sl InitialL}_e(#1)}
\newcommand{\jeInitR}[2]{\hbox{\sl InitialR}_e(#1,#2)}
\newcommand{\jeCut}[4]{\hbox{\sl Cut}_e(#1,#2,#3,#4)}

\newcommand{\cert}{{\tt cert}\xspace}

%--------------------

\newcommand{\true}{\hbox{\sl t}}
\newcommand{\false}{\hbox{\sl f}}

\newcommand{\ntrue}{t^-}
\newcommand{\ptrue}{t^+}
\newcommand{\nfalse}{f^-}
\newcommand{\pfalse}{f^+}
\newcommand{\wedgep}{\wedge^{\!+}}
\newcommand{\wedgen}{\wedge^{\!-}}
\newcommand{\veep}{\vee^{\!+}}
\newcommand{\veen}{\vee^{\!-}}


\newcommand{\andClerk}[4]{{\wedge^{\!-}}(#1,#2,#3,#4)}
\newcommand{\falseClerk}[2]{f_c(#1,#2)}
\newcommand{\orClerk}[3]{{\vee^{\!-}}(#1,#2,#3)}
\newcommand{\allClerk}[3]{\forall(#1,#2,#3)}
\newcommand{\boxClerk}[3]{\square(#1,#2,#3)}
\newcommand{\storeClerk}[4]{\hbox{\sl store}(#1,#2,#3,#4)}

\newcommand{\trueExpert }[1]{{\true_e}(#1)}
\newcommand{\andExpert}[4]{{\wedge^{\!+}}(#1,#2,#3,#4)}
\newcommand{\andExpertLJF}[6]{{\wedge_e}(#1,#2,#3,#4,#5,#6)}
\newcommand{\orExpert  }[4]{{\vee^{\!+}}(#1,#2,#3,#4)}
\newcommand{\someExpert}[4]{\exists(#1,#2,#3,#4)}
\newcommand{\diamondExpert}[4]{\lozenge(#1,#2,#3,#4)}
\newcommand{\initExpert}[2]{\hbox{\sl init}(#1,#2)}
\newcommand{\initrExpert}[1]{\hbox{\sl initR}E(#1)}
\newcommand{\cutExpert}[4]{\hbox{\sl cut}_e(#1,#2,#3,#4)}
\newcommand{\decideExpert}[3]{\hbox{\sl decide}(#1,#2,#3)}
\newcommand{\releaseExpert}[2]{\hbox{\sl release}(#1,#2)}
\newcommand{\decideExpertStar}[5]{\hbox{\sl decide}_e^*(#1,#2,#3,#4,#5)}

\newcommand{\reflClerk}[2]{\blue{T_c(#1,#2)}}
\newcommand{\transClerk}[2]{\blue{4_c(#1,#2)}}
\newcommand{\symmClerk}[2]{\blue{B_c(#1,#2)}}
\newcommand{\euclClerk}[2]{\blue{5_c(#1,#2)}}
\newcommand{\serClerk}[2]{\blue{D_c(#1,#2)}}

\newcommand{\blue}[1]{{\color[rgb]{0,0,1} #1}}
\newcommand{\tupp}[2]{\blue{\langle #1,}#2{\blue{\rangle}}}


\newcommand{\seqneg}[2]{\vdash #1 ; #2}
\newcommand{\seqpos}[3]{\vdash #1 ; #2 ; #3}
\newcommand{\Ncal}{{\cal N}}
\newcommand{\seqnega}[3]{\blue{#1} \vdash #2 ; #3}
\newcommand{\seqposa}[4]{\blue{#1} \vdash #2 ; #3 ; #4}

\newcommand{\mkpos}[1]{\partial\kern -1pt_{\scriptscriptstyle +}\kern -1pt(#1)}
\newcommand{\mkneg}[1]{\partial\kern -1pt_{\scriptscriptstyle -}\kern -1pt(#1)}

\newcommand{\tup}[1]{\langle #1\rangle}

\newcommand{\ra}{\rightarrow}
\newcommand{\args }[2]{(\hbox{\tt args}~#1~#2)}
\newcommand{\lc   }[2]{(\hbox{\tt lc}~#1~#2)}
\newcommand{\apply}[2]{(\hbox{\tt apply}~#1~#2)}
\newcommand{\lidx }[1]{(\hbox{\tt idx}~#1)}
\newcommand{\mapping}[3]{[\![#1\mathbin{|}#2]\!]_{#3}}

\newcommand{\delayop}{\ensuremath{\partial}}
\newcommand{\negdop}{\delayop}
\newcommand{\posdop}{\rotatebox[origin=c]{180}{\delayop}}
%\newcommand{\negd}[1]{\negdop\mkern -2mu\left(#1\right)}
%\newcommand{\posd}[1]{\posdop\mkern -2mu\left(#1\right)}
\newcommand{\negd}[1]{\delayop^-(#1)}
\newcommand{\posd}[1]{\delayop^+(#1)}

% MODAL FOCUSING MACROS
\newcommand{\tr}[2]{\lbrack #1 \rbrack_{#2}}
\newcommand{\mapp}[1]{\tau(#1)}
%\newcommand{\polos}[1]{\lbrack #1 \rbrack}
\newcommand{\polos}[1]{\lfloor #1 \rfloor}
\newcommand{\intlmf}[1]{\mathcal{I}_{F}(#1)}
\newcommand{\intlmfx}[1]{\mathcal{I}^{X}_{F}(#1)}
\newcommand{\intlmfour}[1]{\mathcal{I}_{F}(#1)}
\newcommand{\eqform}{=}
\newcommand{\eqformx}{=}
\newcommand{\intos}[1]{\mathcal{I}_{OS}(#1)}
%\newcommand{\intos}[1]{#1}
\newcommand{\intns}[1]{\mathcal{I}_{NS}(#1)}
\newcommand{\inths}[1]{\mathcal{I}_{HS}(#1)}
\newcommand{\str}[2]{ST_{#2}(#1)}
\newcommand{\nnf}[1]{#1^\circ}
\newcommand{\elements}[1]{\mathcal{L}(#1)}
\newcommand{\trlab}[1]{\lbrack #1 \rbrack}
\newcommand{\trseq}[2]{\lbrack #1 \rbrack_{#2}}
\newcommand{\trf}[1]{\lbrack #1 \rbrack}
\newcommand{\trlf}[2]{\lbrack #1 \rbrack_{#2}}
\newcommand{\trplus}[1]{\lbrack #1 \rbrack^{+}}
\newcommand{\rel}{R}
\newcommand{\ar}{\mathcal{G}}
\newcommand{\wld}{W}
\newcommand{\val}{V}
\newcommand{\m}{\mathcal{M}}
\newcommand{\prop}{\mathcal{P}}
\newcommand{\hp}{\mathcal{H}}
\newcommand{\fl}{\mathcal{F}}
\newcommand{\relfo}{R}
\newcommand{\refl}{refl}
\newcommand{\trans}{trans}
\newcommand{\symm}{symm}
\newcommand{\eucl}{eucl}
\newcommand{\ser}{ser}
\newcommand{\reflf}{T_F}
\newcommand{\transf}{4_F}
\newcommand{\symmf}{B_F}
\newcommand{\euclf}{5_F}
\newcommand{\serf}{D_F}

\newcommand{\refla}{T_a}
\newcommand{\transa}{4_a}
\newcommand{\symma}{B_a}
\newcommand{\eucla}{5_a}
\newcommand{\sera}{D_a}

\newcommand{\dir}{dir_F}
\newcommand{\conn}{conn}
\newcommand{\init}{init}
\newcommand{\initR}{\init_{R}}
\newcommand{\lwedge}{L\wedge}
\newcommand{\rwedge}{R\wedge}
\newcommand{\lvee}{L\vee}
\newcommand{\rvee}{R\vee}
\newcommand{\lbox}{L\square}
\newcommand{\rbox}{R\square}
\newcommand{\ldiamond}{L\lozenge}
\newcommand{\rdiamond}{R\lozenge}
\newcommand{\boxT}{\square_T}
\newcommand{\diamondT}{\lozenge_T}
\newcommand{\boxdiamondD}{\square\lozenge_D}
\newcommand{\impl}{\supset}
\newcommand{\limpl}{L{\impl}}
\newcommand{\rimpl}{R{\impl}}
\newcommand{\lbot}{L\bot}
\newcommand{\logick}{K}
\newcommand{\logicr}{R}
\newcommand{\lab}{\mathcal{L}}
\newcommand\labk {\proofsystem{LS}}
\newcommand\lss {\proofsystem{LS}}
\newcommand\labkF {\proofsystem{LMF}}
%\newcommand\lmf {\hbox{\proofsystem{LMF}\kern-2pt$^a$}\xspace}
\newcommand\lmf {\hbox{\proofsystem{LMF}}}
\newcommand\lmfx {\lmf^{X}}
\newcommand\lmfxos {\lmfx_{OS}}
\newcommand\nlab {\proofsystem{UM}}
\newcommand\mdl {\nlab}
\newcommand\os {OS}
\newcommand\osx {OS^{X}}
\newcommand\dec {\nlab^{d}}
\newcommand\foc {\labkF}
\newcommand\multi {\labkF}
\newcommand\price {PRICE}
\newcommand\aug {\multi^{a}}
\newcommand\labkstarF  {\proofsystem{G3K^*F}}
\newcommand\labr  {\proofsystem{R}}
%\newcommand{\fix}[2]{{\bf FIX}\footnote{{\bf #1:} #2}}

\newcommand{\fix}[2]{

\fbox{\begin{minipage}{40em}
{\bf #1:} #2
\end{minipage}}}

\newcommand{\initf}{init_F}
\newcommand{\initrf}{init_{\rel F}}
\newcommand{\cutf}{cut_F}
\newcommand{\cut}{cut}
\newcommand{\storef}{store_F}
\newcommand{\releasef}{release_F}
\newcommand{\decidef}{decide_F}
\newcommand{\decide}{decide}
\newcommand{\wedgenf}{\wedgen_F}
\newcommand{\veenf}{\veen_F}
\newcommand{\wedgepf}{\wedgep_F}
\newcommand{\veepf}{\veep_F}
\newcommand{\boxf}{\square_F}
\newcommand{\diamondf}{\lozenge_F}
\newcommand{\implf}{{\impl}_F}
\newcommand{\ntruef}{{\ntrue}_F}
\newcommand{\nfalsef}{{\nfalse}_F}
\newcommand{\ptruef}{{\ptrue}_F}
\newcommand{\forallf}{\forall_F}
\newcommand{\existsf}{\exists_F}
\newcommand{\delpf}{\delayop^+_F}
\newcommand{\delnf}{\delayop^-_F}

\newcommand{\inita}{init_{a}}
\newcommand{\initra}{init_{\rel a}}
\newcommand{\cuta}{cut_{a}}
\newcommand{\storea}{store_{a}}
\newcommand{\releasea}{release_{a}}
\newcommand{\decidea}{decide_{a}}
\newcommand{\wedgena}{\wedgen_{a}}
\newcommand{\veena}{\veen_{a}}
\newcommand{\wedgepa}{\wedgep_{a}}
\newcommand{\veepa}{\veep_{a}}
\newcommand{\boxa}{\square_{a}}
\newcommand{\diamonda}{\lozenge_{a}}
\newcommand{\impla}{{\impl}_{a}}
\newcommand{\ntruea}{{\ntrue}_{a}}
\newcommand{\nfalsea}{{\nfalse}_{a}}
\newcommand{\ptruea}{{\ptrue}_{a}}
\newcommand{\foralla}{\forall_{a}}
\newcommand{\existsa}{\exists_{a}}
\newcommand{\delpa}{\delayop^+_{a}}
\newcommand{\delna}{\delayop^-_{a}}

\newcommand{\initk}{init_K}
\newcommand{\initrk}{init_{\rel K}}
\newcommand{\cutk}{cut_K}
\newcommand{\storek}{store_K}
\newcommand{\releasek}{release_K}
\newcommand{\decidek}{decide_K}
\newcommand{\wedgenk}{\wedgen_K}
\newcommand{\veenk}{\veen_K}
\newcommand{\wedgepk}{\wedgep_K}
\newcommand{\veepk}{\veep_K}
\newcommand{\boxk}{\square_K}
\newcommand{\diamondk}{\lozenge_K}
\newcommand{\implk}{{\impl}_K}
\newcommand{\ntruek}{{\ntrue}_K}
\newcommand{\nfalsek}{{\nfalse}_K}
\newcommand{\ptruek}{{\ptrue}_K}
\newcommand{\forallk}{\forall_K}
\newcommand{\existsk}{\exists_K}
\newcommand{\delpk}{\delayop^+_K}
\newcommand{\delnk}{\delayop^-_K}
\newcommand{\bxed}[1]{#1^{\square}}
\newcommand{\dmed}[1]{#1^{\lozenge}}

\newcommand{\delp}[1]{{#1}^{\delayop^{+}}}
\newcommand{\axiom}{G}
\newcommand{\fv}[1]{FV(#1)}
\newcommand{\unpol}[1]{\hat{#1}}

\newcommand{\krule}{\square_{K}}
\newcommand{\trule}{\lozenge_{T}}
\newcommand{\drule}{\lozenge_{D}}
\newcommand{\kfourrule}{\square_{K4}}
\newcommand{\kfiverule}{\square_{K45}}

\newcommand{\checkers}{\texttt{Checkers}}
\newcommand\lmfm {\hbox{\proofsystem{LMF$_m$}}}
\newcommand\lmfs {\lmfstar}
\newcommand\nss {\hbox{\proofsystem{NS}}}
\newcommand\pt {\hbox{\proofsystem{PT}}}
%\newcommand\os {\hbox{\proofsystem{OS}}}

\newcommand{\Gccon}[2]{\mathcal N\{#1\}\{#2\}}
\newcommand{\Gcon}[1]{\mathcal N\{#1\}}
\def\minidia{\hbox{$\scriptscriptstyle\lozenge$}} % minidiamond
\def\diarule#1{{#1}^{\minidia}}


\newcommand{\contr}{contr}

\newcommand\lmfstar {\hbox{$LMF_{*}$}}

\newcommand{\lft}{\texttt{left}}
\newcommand{\rgt}{\texttt{right}}
\newcommand{\diaind}{\texttt{diaind}}


